Planted Hitting Set Recovery in Hypergraphs

In various application areas, networked data is collected by measuring interactions involving some specific set of core nodes. This results in a network dataset containing the core nodes along with a potentially much larger set of fringe nodes that all have at least one interaction with a core node. In many settings, this type of data arises for structures that are richer than graphs, because they involve the interactions of larger sets; for example, the core nodes might be a set of individuals under surveillance, where we observe the attendees of meetings involving at least one of the core individuals. We model such scenarios using hypergraphs, and we study the problem of core recovery: if we observe the hypergraph but not the labels of core and fringe nodes, can we recover the "planted" set of core nodes in the hypergraph? We provide a theoretical framework for analyzing the recovery of such a set of core nodes and use our theory to develop a practical and scalable algorithm for core recovery. The crux of our analysis and algorithm is that the core nodes are a hitting set of the hypergraph, meaning that every hyperedge has at least one node in the set of core nodes. We demonstrate the efficacy of our algorithm on a number of real-world datasets, outperforming competitive baselines derived from network centrality and core-periphery measures.

==> fig-tikz/hypergraph.tex <==
a

==> proofs.tex <==
%!TEX root = main.tex 

\section{Proofs}\label{app:proofs}

\xhdr{\cref{lem:upper} sub-proof, Fact 1}
By the definition of a sunflower, the sets $X_{t,i}\setminus Y_t$ are
pairwise disjoint for $i = 1, 2,\ldots, k+ 1$. Thus, if $C$ is a set of size
at most $k$ that doesn't contain any nodes of $Y_t$, then it must be disjoint
from at least one of the sets $X_{t,i}$, and hence it can't be a hitting set for
$H_{t-1}$.
%
The definition of $H_t$ is as follows: starting from $H_{t-1}$, we remove the hyperedges
$X_{t,1}, X_{t,2},\ldots, X_{t,k+1}$ and add the hyperedge $Y_t$. Since
$H_{t-1}$ and $H_{t}$ are hypergraphs on the same node sets, their respective
collections of hitting sets $C(H_{t-1})$ and $C(H_{t})$ are also over the same
sets of elements. 
% and hence it makes sense to compare them.

\xhdr{\cref{lem:upper} sub-proof, Fact 2}
Let $C\in \mathcal{C}(H_{t-1})$. Then by part (1), it must intersect $Y_t$. Since
$Y_t$ is the only hyperedge in $H_t$ but not $H_{t-1}$, it follows that $C$ is a
hitting set for $H_t$, and hence $C\in \mathcal{C}(H_t)$. Conversely, let
$C'\in \mathcal{C}(H_t)$. Since $Y_t\subset X_{t,i}$ for $i = 1, 2,\ldots, k+1$,
it must be that $C_0$ intersects each $X_{t,i}$. Since
$X_{t,1}, X_{t,2},\ldots, X_{t,k+1}$ are the only hyperedges in $H_{t-1}$ but not $H_t$, it
follows that $C\in \mathcal{C}(H_{t-1})$.  Thus,
$\mathcal{C}(H_{t-1}) \subset \mathcal{C}(H_t) \subset \mathcal{C}(H_{t-1})$, and so they are equal as sets.

\xhdr{\cref{lem:outside}}
%
We perform a pruning of $C$ as follows. Check whether there exists a node
$w$ with $C \setminus \{w\}$ still being a hitting set of smaller
cardinality. If this is the case, update $C$ to $C \setminus \{w\}$ and continue
pruning. Upon termination, the remaining set is a minimal hitting set
$C' \subseteq C$. Clearly, $\lvert C' \rvert \leq \lvert C \rvert$ so that $C'\subset \UsizeC$.
However, $u \in U(\lvert C \rvert)$ since $(u,v_1,\ldots,v_i)$ is a hyperedge where $v_1,\ldots,v_i\notin C$.

\xhdr{\cref{lem:interior}}
%
Since $v_1,\ldots,v_i$ are in the interior of $C$,
$C_0=C\setminus\{v_1,\ldots,v_i\}$ is a hitting set as well. Now perform pruning
on $C_0$ as in the previous proof, the output of which is $C'\subset C_0$, and
since clearly $|C'|\leq \lvert C \rvert$, we must have that $C'\subset \UsizeC$.
Clearly $u$ was not deleted during pruning since $(u,v_1,\ldots,v_i)$ is a
hyperedge with $v_1,\ldots,v_i\notin C$, so that $u\in C'\subset \UsizeC$.

\xhdr{\cref{lem:independence}}
We follow a proof technique common in the combinatorics literature~\cite{Kostochka-2014-independent}.
Let $z = \binom{\lvert G \rvert}{k}$,
$S_1,\ldots,S_{z}$ the size-$k$ subsets of vertices of $G$,
and $X_i$ an indicator random variable for $S_i$ being an independent set of $G$,
so $X_i = 1$ only happens when all $\binom{k}{r}$ possible hyperedges among 
the vertices of $S_i$ do not appear in the hyperedge set of $G$.
Note that this happens with probability
$(1-p)^{\binom{k}{r}}=(1-p)^{\frac{k\cdot\cdot\cdot\cdot(k-r+1)}{r!}}\leq(1-p)^{\frac{k(k-r+1)}{r!}}$. Thus,
\begin{eqnarray*}
  \textstyle \textnormal{Pr}(\alpha(G)\geq k)
  &=& \textstyle
  \text{Pr}(\sum_iE(X_i) \geq 1) 
    \leq \sum_iE(X_i)
    = \binom{n}{k}(1-p)^{\binom{k}{r}}\\
  &\leq& \textstyle
    \binom{n}{k}(1-p)^{\frac{k(k-r+1)}{r!}}
\leq n^k\left((1-p)^{(k-r+1)/r!}\right)^k\\
&\leq& \textstyle
(ne^{-p(k-r+1)/r!})^k\\
&=&n^{-\frac{1}{2}\left(\frac{3r!\ln n}{2p}+(r-1)\right)}
\end{eqnarray*}
so that
$\textnormal{Pr}(\alpha(G)<k)\geq 1-n^{-\frac{1}{2}\left(\frac{3r!\ln n}{2p}+(r-1)\right)}$,
as desired.


==> reproducibility.tex <==
%!TEX root = main.tex

\section*{Reproducibility}

\begin{figure*}[t!!]
\lstdefinelanguage{Julia}%    
{morekeywords={abstract,break,case,catch,const,continue,do,else,elseif,end,export,false,for,function,immutable,import,importall,if,in,macro,module,otherwise,quote,return,switch,true,try,type,typealias,using,while},%
sensitive=true,%
alsoother={$},%
morecomment=[l]\#,%
morecomment=[n]{\#=}{=\#},%
morestring=[s]{"}{"},%
morestring=[m]{'}{'},% 
}[keywords,comments,strings]%
\lstset{%
language         = Julia,
basicstyle       = \footnotesize \ttfamily,
keywordstyle     = \bfseries\color{blue},
stringstyle      = \color{magenta},
commentstyle     = \color{orange},                                                                                                                                         
showstringspaces = false,
numbers=left,                                                                                                                                                       
}
\scalebox{1.0}{\lstinputlisting{UMHS.jl}}
\caption{The union of minimal hitting sets algorithm. 
The inputs are a vector $a$ of all nodes in the order in which they appear in all 
hyperedges and a vector $b$ of the number of nodes in each of those hyperedges. 
Lines 3--9 recreate the hypergraph structure from those two vectors. 
Lines 12--18 run \cref{alg:greedy}. 
Lines 20--35 remove nodes that do not intersect with other hyperedges, 
thus beginning to prune the hitting set with the goal of maintaining minimality.
 Lines 37--49 finish the pruning. 
 Lines 53--55 sort the output union of minimal hitting sets by degree, and also sort the remaining nodes by degree.}
\label{fig:julia_umhs}
\end{figure*}

\subsection*{Software}

Our code was written in Julia version 1.1. The main computational kernel is the
union of minimal hitting sets algorithm (\cref{alg:UMHS}), and we provide the
code below in \cref{fig:julia_umhs}.

We will release all of our software upon publication. For now, we do not
include it to preserve anonymity.

\subsection*{Data}

All data that we used is publicly available, with partial exception
for the Avocado email dataset. The Avocado dataset is available for
academic purposes but not commerical ones: \url{https://catalog.ldc.upenn.edu/LDC2015T03}.

We will release processed formats of the data upon publication that work with our software. 
Again, we do not post them now in an effort to preserve anonymity. 



\subsection*{Full proof of \cref{lem:lower}}

Here we present the full proof of \cref{lem:lower}. This lemma was
stated without a complete proof by Damaschke~\cite[Proposition 9]{Damaschke-2006-parameterized}.

For a parameter $b$, consider a graph $\Gamma_b$ that consists of $b$ disjoint
complete $b$-ary trees of depth $r$. We will refer to the roots of the $b$ trees
in $\Gamma_b$ as the root nodes of $\Gamma_b$, and to the leaves of the trees in
$\Gamma_b$ as leaf nodes. Let $T_b$ be the hypergraph on the node set of
$\Gamma_b$ whose hyperedges consist of all root-to-leaf paths in $\Gamma_b$,
from the root of one of the $b$ trees in $\Gamma_b$ to a leaf of the
corresponding tree (the example of $T_2$ for $r=3$ is in \cref{fig:trees}). All
edges in $G$ have size $r$.  Let $\lambda$ be any function that maps nodes of
$\Gamma_b$ to numbers in $\{1, 2, . . . ., b\}$ with the following properties:
(i) $\lambda$ is a bijection from the roots of $\Gamma_b$ to $\{1, 2, \ldots, b\}$;
and (ii) for each non-leaf node $v$ in $\Gamma_b$, $\lambda$ is a
bijection from the children of $v$ to $\{1, 2, . . . ., b\}$. For each node $v$,
we will call $\lambda(v)$ its label (with respect to $\lambda$), and we will say
that $\lambda$ is a consistent labeling if it satisfies (i) and (ii).  Let
$v^{*}_{\lambda}$ be unique leaf node for which all the nodes on the
root-to-leaf path have the label $b$.

For a consistent labeling $\lambda$, let $C_\lambda$ be the set of all nodes $v$
satisfying two properties: (i) $\lambda(u) = b$ for all nodes $u$ on the unique
path from a root of $\Gamma_b$ to $v$ (other than $v$ itself), and (ii)
$\lambda(v) \neq b$. Let $C^{*}_{\lambda} = C_\lambda\cap\{v^{*}_{\lambda}\}$.
We observe the following two facts.
\begin{enumerate}
\item For every consistent labeling $\lambda$, the set $C^{*}_{\lambda}$ is a
  minimal hitting set for $T_b$.
\item Every node v of $T_b$ belongs to at least one set of the form
  $C^{*}_{\lambda}$ for some consistent labeling $\lambda$.
\end{enumerate}
To prove (1), we claim that $C^{*}_{\lambda}$ is a hitting set.
Consider any hyperedge $X$ of $T_b$, consisting of a root-to-leaf path $P$ in
$\Gamma_b$. If all nodes on $P$ have label $b$, then the leaf node of $P$ is
$v^{*}_{\lambda}$, and hence $X$ intersects $C^{*}_{\lambda}$. Otherwise,
consider the first node $v$ on the path $P$ that has a label unequal to
$b$. Thus, $v \in  C^{*}_{\lambda}$, and again $X$ intersects
$C^{*}_{\lambda}$ and $C^{*}_{\lambda}$ is a hitting set. We now argue that it is minimal.
If we delete $v^{*}_{\lambda}$ from $C^{*}_{\lambda}$, then
$C^{*}_{\lambda}\setminus \{v^{*}_{\lambda}\}$ would be disjoint from the
hyperedge $X$ consisting of the root-to-leaf path to $v^{*}_{\lambda}$. If we
delete some other $v^{*}_{\lambda}$, then a hyperedge $X$ that passes through
$v$ does not pass through any other node of $C^{*}_{\lambda}$ on its way from
root to leaf, and so $C^{*}_{\lambda}\setminus \{v\}$ would be disjoint from
$X$.

To prove (2), we simply choose any consistent labeling $\lambda$ such that
$\lambda(u) = b$ for all nodes $u$ on the unique path from a root of $\Gamma_b$
to $v$ (other than $v$ itself), and $\lambda(v) \neq b$.

Now, we consider the size of a set of the form $C^{*}_{\lambda}$. Since
$C^{*}_{\lambda}$ contains $b - 1$ nodes from each of the first $r - 1$ levels
of the trees in $\Gamma_b$, and $b$ from the lowest level, we have
\[
\lvert C^{*}_{\lambda} \rvert = (r - 1)(b - 1) + b.
\]

We define $k = (r - 1)(b - 1) + b$. Since each set $C^{*}_{\lambda}$ is a
minimal hitting set of size $k$, from (2) we see that the union $U(k)$ of all
minimal hitting sets of size $k$ is the entire node set of $T_b$.

The number of nodes in $T_b$ is greater than $b^r$, and hence
%
$\lvert U(k) \rvert > b^r$.
%
Since $k \leq br$, we have that $\lvert U(k) \rvert > b^r\geq (k/r)^r = r^{-r}k^r$.
